Automated Detection of Typed Links in Issue Trackers

Stakeholders in software projects use issue trackers like JIRA to capture and manage issues, including requirements and bugs. To ease issue navigation and structure project knowledge, stakeholders manually connect issues via links of certain types that reflect different dependencies, such as Epic-, Block-, Duplicate-, or Relate- links. Based on a large dataset of 15 JIRA repositories, we study how well state-of-the-art machine learning models can automatically detect common link types. We found that a pure BERT model trained on titles and descriptions of linked issues significantly outperforms other optimized deep learning models, achieving an encouraging average macro F1-score of 0.64 for detecting 9 popular link types across all repositories (weighted F1-score of 0.73). For the specific Subtask- and Epic- links, the model achieved top F1-scores of 0.89 and 0.97, respectively. Our model does not simply learn the textual similarity of the issues. In general, shorter issue text seems to improve the prediction accuracy with a strong negative correlation of -0.70. We found that Relate-links often get confused with the other links, which suggests that they are likely used as default links in unclear cases. We also observed significant differences across the repositories, depending on how they are used and by whom.

==> figures/LT_confidence.tex <==
\begin{figure}[h!]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[scale=0.36]{pictures/LT_Confidence_JiraEcosystem.png}
    \caption{JiraEcosystem}
    \label{fig:LTConfJiraEcosystem}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[scale=0.36]{pictures/LT_Confidence_MariaDB.png}
    \caption{MariaDB}
    \label{fig:LTConfMariaDB}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[scale=0.36]{pictures/LT_Confidence_Qt.png}
    \caption{Qt}
    \label{fig:LTConfQt}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[scale=0.36]{pictures/LT_Confidence_Sakai.png}
    \caption{Sakai}
    \label{fig:LTConfSakai}
\end{subfigure}
\caption{Violinplots of the confidence of the classifier of four repositories.}
\label{fig:LTConfidence}
\end{figure}

==> figures/LT_confusion_matrix.tex <==
\begin{figure*}[htp]
\centering
\includegraphics[scale=0.43]{pictures/confmats.png}
    \caption{Normalized confusion matrices for each repository. Rows are sorted by support of link type, meaning the majority class is always the first row.}
\label{fig:LTConfMat}
\end{figure*}

==> figures/LT_performance.tex <==
\begin{figure}[htp]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[scale=0.43]{pictures/LT_F1.png}
    \caption{F1 score of the classifier.}
    \label{fig:LTF1}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[scale=0.43]{pictures/LT_Share.png}
    \caption{Share of link type in a repository.}
    \label{fig:LTPart}
\end{subfigure}
\caption{Boxplots of the performance of the classifier on common link types across the repositories sorted by median F1 score.}
\label{fig:LTPerformance}
\end{figure}

==> old.tex <==
% \subsection{Embeddings visualized with t-SNE / PCA}

% color_cat = {
%     'General Relation': 'lightseagreen', 
%     'Composition': 'dodgerblue',
%     'Duplication': 'gold',
%     'Temporal/Causal': 'purple',
%     'Workflow': 'black'}
    
% Figure~\ref{fig:LinkCatEmbedding} shows the embeddings after performing tsne on them to plot them in lower dimensions. We see that some separation is possible. Composition and General Relation are almost always very separate, whereas Duplication, Temporal / Causal and Workflow have an overlap.
% \input{figures/embed_tsne_3}
% \input{figures/embed_tsne_2}
% Interestingly enough tsne does not seem to find a decent visualization for Apache, which might be due to the size of the project and the many subprojects.

% \subsection{Embeddings for Link Category Prediction}
% We used the resulting embeddings to predict the link category of the independent test set.
% Table~\ref{tab:Results} shows the results of using an SVM to predict the categories per project.
% % \input{tables/results_svm}
% We see that the embeddings are useful for predicting the different link categories.

% Figure~\ref{fig:SVMConfMats} shows the confusion matrices divided by the number of instances per class of the test set. Thus, the diagonal is the recall per class.
% \begin{figure*}
%         %  \centering
%         \includegraphics[width=0.95\textwidth]{pictures/SCCNN_cat_confmats.png}
%       \caption{Confusion Matrices of SVM approach to distinguish link types}\label{fig:SVMConfMats}
% \end{figure*}
% We observe that some projects have a very overlapping \textit{General Relation} usages, such as Jiraecosystem, Sakai, IntelDAOS, Sonatype, and Spring.
% \textit{Composition} was the best class to distinguish except for Jira.\\
% \textbf{TO-DO: Do fine-grained error analysis.}

% Table~\ref{tab:LinkCatStats} shows the distribution of link categories across the projects
% \input{tables/project_link_cat_distribution}

\section{OLD Results}
In this section we present the results of the link type classification and analyze them for each project. We also analyze the errors of the classifier.
As there is no large scale link detection paper, we calculated a random baseline which assigns a label based on the distribution of the labels in the data set.
Table~\ref{tab:BaselineImproveLT} shows how much the accuracy and macro F1 score of our classification improved in comparison to the random baseline.
\input{tables/results_baseline_improve_LT}

\clearpage
\subsection{Apache}
Apache overall has 21 link types and 242823 links.
After cleaning up link types like ``Reference'' and ``Related'', mapping them together, as well as ``Blocker'' and ``Blocked'', and ``dependent'', ``Dependent'', and ``Dependency'', we arrive at 15 link types.
We only predict on 12 of them, as ``Parent-Child'' (2065), ``Fix'' (533), and ``Bonfire Testing'' (2) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on Apache links.}\label{tab:ResultsApache}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{good} Relate       &   0.633047 &  0.535501 &  0.580203 &  13901 \\
\rowcolor{subpar} Cause        &   0.024684 &  0.080913 &  0.037827 &    482 \\
\rowcolor{moderate} Duplicate    &   0.378484 &  0.367040 &  0.372675 &   4994 \\
\rowcolor{moderate} Incorporate  &   0.331585 &  0.273164 &  0.299553 &   2083 \\
\rowcolor{subpar} Clone        &   0.122825 &  0.143027 &  0.132159 &    839 \\
\rowcolor{subpar} Supercede    &   0.047729 &  0.134522 &  0.070458 &    617 \\
\rowcolor{subpar} Require      &   0.056263 &  0.150997 &  0.081980 &    702 \\
\rowcolor{verygood} Subtask      &   0.931425 &  0.927926 &  0.929672 & 15706 \\
\rowcolor{moderate} Block        &   0.405641 &  0.203573 &  0.271095 &   2967 \\
\rowcolor{subpar} Depend       &   0.223801 &  0.048818 &  0.080153 &   2581 \\
\rowcolor{subpar} Breaks       &   0.061028 &  0.248555 &  0.097995 &    865 \\
\rowcolor{verygood} Epic         &   0.956354 &  0.963362 &  0.959845 &   2320 \\
\hline
accuracy     & \multicolumn{4}{r|}{0.581559}   \\
macro avg    &   0.347739 &  0.339783 &  0.326134 &  48057 \\
weighted avg &   0.629385 &  0.581559 &  0.597309 &  48057 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsApache} shows the result of an SVM trained on the links of the Apache project. 
We observe that the detection works well on ``Epic'' and ``Subtask'', and is also able to predict ``Relate'' fairly well. ``Duplicate'', ``Incorporate'', and ``Block'' are not good and the rest is sub-par.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_apache_confmat.png}
\caption{Confusion Matrix in percent of Apache.}\label{fig:ConfMatApache}
\end{figure}
Figure~\ref{fig:ConfMatApache} shows the confusion matrix. 
We observe that the classifier tends to predict ``Relate'', for most types, except ``Subtask'' and ``Epic''. Apache is a very heterogenous project, its subprojects are rather diverse and almost projects on their own, which could explain the struggles of the classifier. In this case it might make sense to apply the link detection per subproject.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_apache_test_umap_2.png}
\caption{UMAP of the test data embeddings of Apache.}\label{fig:UMAPApache}
\end{figure}
Figure~\ref{fig:UMApApache} shows the UMAP on the embeddings of the test set, the trend found during classification is also clearly visible here.

k-Means found 7 as the optimal number of clusters, but there is no clear assignment of link types to specific clusters, except for ``Epic'' and ``Subtask''
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_apache_test_ltcomp.png}
    \caption{kMeans with optimal k Apache}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_apache_test_acc_ltcomp.png}
    \caption{kMeans with accurate k Apache}
\end{subfigure}
\caption{kMeans of Apache.}\label{fig:kMeansApache}
\end{figure}

\textbf{\large{TO-DO: SUBPROJECT WISE CLASSIFICATION!!!!!}}

\clearpage
\subsection{Hyperledger}
Hyperledger overall has 8 link types and 16225 links.
We only predict on 6 of them, as ``Split'' (74), and ``Bonfire Testing'' (7) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on Hyperledger links.}\label{tab:ResultsHyperledger}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{moderate} Block        &   0.521429 &  0.268382 &  0.354369 &  272 \\
\rowcolor{verygood} Epic         &   0.960311 &  0.983267 &  0.971654 &  1255 \\
\rowcolor{good} Relate       &   0.763797 &  0.633700 &  0.692693 &   546 \\
\rowcolor{subpar} Duplicate    &   0.129129 &  0.387387 &  0.193694 &   111 \\
\rowcolor{moderate} Clone        &   0.263158 &  0.376344 &  0.309735 &    93 \\
\rowcolor{verygood} Subtask      &   0.936723 &  0.870798 &  0.902559 &   952 \\
\hline
accuracy     & \multicolumn{4}{r|}{0.792815} \\
macro avg    &   0.595758 &  0.586646 &  0.570784 &  3229 \\
weighted avg &   0.834506 &  0.792815 &  0.806307 &  3229 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsHyperledger} shows the result of an SVM trained on the links of the Hyperledger project. 
We observe that the detection works well on ``Epic'', ``Relate'' and ``Subtask''.
For ``Duplicate'' the detection achieves sub-par results.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_hyperledger_test_confmat.png}
\caption{Confusion Matrix in percent of Hyperledger.}\label{fig:ConfMatHyperledger}
\end{figure}
Figure~\ref{fig:ConfMatHyperledger} shows the confusion matrix. 
We observe that the classifier tends to predict ``Block'' for ``Relate'', ``Duplicate'', and ``Clone''. ``Relate'' is fairly unique. ``Duplicate'' are often mistaken for ``Block'' and ``Relate''.
``Clone'' is often mistaken for ``Duplicate'' followed by ``Block''.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_hyperledger_test_umap_2.png}
\caption{UMAP of the test data embeddings of Hyperledger.}\label{fig:UMAPHyperledger}
\end{figure}
Figure~\ref{fig:UMAPHyperledger} shows the UMAP on the embeddings of the test set.

k-Means found 4 as the optimal number of clusters, where ``Block'', ``Clone'', and ``Duplicate'' share a cluster, whereas ``Epic'', ``Relate'', and ``Subtask'' all have their own clusters.
With the acutal number of link types as clusters ``Block'', ``Clone'', and ``Duplicate'' 

\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_hyperledger_test_ltcomp.png}
    \caption{kMeans with optimal k Hyperledger}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_hyperledger_test_acc_ltcomp.png}
    \caption{kMeans with accurate k Hyperledger}
\end{subfigure}
\caption{kMeans of Hyperledger.}\label{fig:kMeansHyperledger}
\end{figure}

\subsection{IntelDAOS}
IntelDAOS was too small.

\clearpage
\subsection{JFrog}
JFrog overall has 11 link types and 3206 links.
After cleaning up link types like ``Gantt End to End'' and ``Finish-to-Finish link (WBSGantt)'', mapping them together, we arrive at 10 link types.
We only predict on 6 of them, as ``Clone'' (20), ``finish-finish'' (5), ``finish-start'' (3), and ``start-start'' (1) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on JFrog links.}\label{tab:ResultsJFrog}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{verygood} Subtask      &   0.965368 &  0.910204 &  0.936975 &  245 \\
\rowcolor{moderate} Relate       &   0.420290 &  0.524096 &  0.466488 &  166 \\
\rowcolor{moderate} Depend       &   0.571429 &  0.173913 &  0.266667 &   46 \\
\rowcolor{moderate} Duplicate    &   0.354167 &  0.395349 &  0.373626 &  129 \\
\rowcolor{subpar} Trigger      &   0.153846 &  0.097561 &  0.119403 &   41 \\
\rowcolor{subpar} Incorporate  &   0 &  0 &  0 &    9 \\
\hline
accuracy     &   \multicolumn{4}{r|}{0.586478} \\
macro avg    &   0.410850 &  0.350187 &  0.360526 &  636 \\
weighted avg &   0.604661 &  0.586478 &  0.585465 &  636 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsJFrog} shows the result of an SVM trained on the links of the JFrog project. 
We observe that the detection works well on ``Subtask'' and fairly well for ``Relate'', ``Depend'', and ``Duplicate''.
For ``Trigger'' and ``Incorporate'' the detection achieves sub-par results.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_jfrog_test_confmat.png}
\caption{Confusion Matrix in percent of JFrog.}\label{fig:ConfMatJFrog}
\end{figure}
Figure~\ref{fig:ConfMatJFrog} shows the confusion matrix. 
We observe that the classifier tends to predict ``Relate'' and ``Duplicate'' for most types, except ``Subtask''. ``Incoporate'' is also falsely assigned to ``Relate'' and ``Duplicate'' links.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_jfrog_test_umap_2.png}
\caption{UMAP of the test data embeddings of JFrog.}\label{fig:UMAPJFrog}
\end{figure}
Figure~\ref{fig:UMAPJFrog} shows the UMAP on the embeddings of the test set.

k-Means found 4 as the optimal number of clusters.
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_jfrog_test_ltcomp.png}
    \caption{kMeans with optimal k JFrog}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_jfrog_test_acc_ltcomp.png}
    \caption{kMeans with accurate k JFrog}
\end{subfigure}
\caption{kMeans of JFrog.}\label{fig:kMeansJFrog}
\end{figure}

\clearpage
\subsection{Jira}
Jira overall has 19 link types and 98122 links.
After cleaning up link types like ``Split'' and ``Issue Split'', mapping them together, as well as ``Reference'', ``Relate'', and ``Related'', we arrive at 14 link types.
We only predict on 7 of them, as ``Block'' (950), ``Derive'' (505), ``Supercede'' (472), ``Breaks'' (355), ``Bonfire Testing'' (216), ``Split'' (168), ``Fix'' (54), ``Depend'' (51), and ``Follow'' (42) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on Jira links.}\label{tab:ResultsJira}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{subpar} Clone        &   0.063158 &  0.192090 &  0.095061 &    531 \\
\rowcolor{subpar} Cause        &   0.078431 &  0.174387 &  0.108199 &    367 \\
\rowcolor{good} Duplicate    &   0.739424 &  0.407119 &  0.587322 &   4270 \\
\rowcolor{verygood} Relate       &   0.875690 &  0.863567 &  0.869586 &  12497 \\
\rowcolor{subpar} Incorporate  &   0.246269 &  0.251908 &  0.249057 &    524 \\
\rowcolor{good} Detail       &   0.404034 &  0.638522 &  0.530702 &    379 \\
\rowcolor{good} Subtask      &   0.712941 &  0.613360 &  0.659412 &    494 \\
\hline
accuracy     &   \multicolumn{4}{r|}{0.719494} \\
macro avg    &   0.402850 &  0.460136 &  0.442763 &  19062 \\
weighted avg &   0.777278 &  0.719494 &  0.740880 &  19062 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsJira} shows the result of an SVM trained on the links of the Jira project. 
We observe that the detection works well on ``Relate''. It is also able to detect ``Duplicate'', ``Detail'' and ``Subtask''. For ``Clone'', ``Cause'', and ``Incorporate'' the detection achieves sub-par results.
This might be correlated to the amount of ``Relate'' links in this data set.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_jira_confmat.png}
\caption{Confusion Matrix in percent of Jira.}\label{fig:ConfMatJira}
\end{figure}
Figure~\ref{fig:ConfMatJira} shows the confusion matrix. 

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_jira_test_umap_2.png}
\caption{UMAP of the test data embeddings of Jira.}\label{fig:UMAPJira}
\end{figure}
Figure~\ref{fig:UMAPJira} shows the UMAP on the embeddings of the test set.

k-Means found 4 as the optimal number of clusters.
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_jira_test_ltcomp.png}
    \caption{kMeans with optimal k Jira}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_jira_test_acc_ltcomp.png}
    \caption{kMeans with accurate k Jira}
\end{subfigure}
\caption{kMeans of Jira.}\label{fig:kMeansJira}
\end{figure}

\clearpage
\subsection{JiraEcosystem}
JiraEcosystem overall has 18 link types and 10911 links.
After cleaning up link types like ``Blocks'' and ``Blocker'', mapping them together, as well as ``Epic'' and ``Epic-Relation'', ``Relate'' and ``Reference'', and ``Bonfire testing'' and ``Bonfire Testing'', we arrive at 13 link types.
We only predict on 10 of them, as ``Follow'' (87), ``Precede'' (7), and ``Bonfire Testing'' (99) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on JiraEcosystem links.}\label{tab:ResultsJiraEcosystem}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{subpar} Clone        &   0.040000 &  0.114286 &  0.059259 &    35 \\
\rowcolor{subpar} Cause        &   0.116883 &  0.130435 &  0.123288 &    69 \\
\rowcolor{subpar} Block        &   0.151724 &  0.180328 &  0.164794 &   122 \\
\rowcolor{good} Relate       &   0.631929 &  0.550193 &  0.588235 &   518 \\
\rowcolor{moderate} Duplicate    &   0.717391 &  0.366667 &  0.405294 &   360 \\
\rowcolor{verygood} Subtask      &   0.893365 &  0.868664 &  0.880841 &   434 \\
\rowcolor{subpar} Incorporate  &   0.133333 &  0.200000 &  0.160000 &    40 \\
\rowcolor{verygood} Epic         &   0.971831 &  0.969880 &  0.970854 &   498 \\
\rowcolor{subpar} Split        &   0.057692 &  0.093750 &  0.071429 &    32 \\
\rowcolor{subpar} Depend       &   0.089744 &  0.388889 &  0.145833 &    36 \\
\hline
accuracy      &   \multicolumn{4}{r|}{0.623601} \\
macro avg    &   0.380389 &  0.386309 &  0.364983 &  2144 \\
weighted avg &   0.697611 &  0.623601 &  0.648229 &  2144 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsJiraEcosystem} shows the result of an SVM trained on the links of the JiraEcosystem project. 
We observe that the detection works well on ``Epic'' and ``Subtask''.
For ``Relate'' the detection works also well, and moderate for ``Duplicate''. For ``Clone'', ``Cause'', ``Block'', ``Incorporate'', ``Split'', and ``Depend'' the detection achieves sub-par results.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_jiraecosystem_test_confmat.png}
\caption{Confusion Matrix in percent of JiraEcosystem.}\label{fig:ConfMatJiraEcosystem}
\end{figure}
Figure~\ref{fig:ConfMatJiraEcosystem} shows the confusion matrix.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_jiraecosystem_test_umap_2.png}
\caption{UMAP of the test data embeddings of JiraEcosystem.}\label{fig:UMAPJiraEcosystem}
\end{figure}
Figure~\ref{fig:UMAPJiraEcosystem} shows the UMAP on the embeddings of the test set.

k-Means found 5 as the optimal number of clusters.
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_jiraecosystem_test_ltcomp.png}
    \caption{kMeans with optimal k JiraEcosystem}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_jiraecosystem_test_acc_ltcomp.png}
    \caption{kMeans with accurate k JiraEcosystem}
\end{subfigure}
\caption{kMeans of JiraEcosystem.}\label{fig:kMeansJiraEcosystem}
\end{figure}

\clearpage
\subsection{MariaDB}
MariaDB overall has 8 link types and 14618 links.
We only predict on 7 of them, as ``Split'' (22) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on MariaDB links.}\label{tab:ResultsMariaDB}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{moderate} Cause        &   0.310345 &  0.305085 &  0.307692 &   177 \\
\rowcolor{good} Incorporate  &   0.510309 &  0.505102 &  0.507692 &   196 \\
\rowcolor{good} Subtask      &   0.700637 &  0.578947 &  0.634006 &   190 \\
\rowcolor{good} Block        &   0.674121 &  0.602857 &  0.636501 &   350 \\
\rowcolor{moderate} Duplicate    &   0.204276 &  0.309353 &  0.246066 &   278 \\
\rowcolor{verygood} Relate       &   0.784287 &  0.742335 &  0.762735 &  1533 \\
\rowcolor{verygood} Epic         &   0.914286 &  0.979592 &  0.945813 &   196 \\
\hline
accuracy     &  \multicolumn{4}{r|}{0.647260} \\
macro avg    &   0.585466 &  0.574753 &  0.577215 &  2920 \\
weighted avg &   0.672026 &  0.647260 &  0.657624 &  2920 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsMariaDB} shows the result of an SVM trained on the links of the MariaDB project. 

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_mariadb_test_confmat.png}
\caption{Confusion Matrix in percent of MariaDB.}\label{fig:ConfMatMariaDB}
\end{figure}
Figure~\ref{fig:ConfMatMariaDB} shows the confusion matrix.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_mariadb_test_umap_2.png}
\caption{UMAP of the test data embeddings of MariaDB.}\label{fig:UMAPMariaDB}
\end{figure}
Figure~\ref{fig:UMAPMariaDB} shows the UMAP on the embeddings of the test set.

k-Means found 5 as the optimal number of clusters.
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_mariadb_test_ltcomp.png}
    \caption{kMeans with optimal k MariaDB}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_mariadb_test_acc_ltcomp.png}
    \caption{kMeans with accurate k MariaDB}
\end{subfigure}
\caption{kMeans of MariaDB.}\label{fig:kMeansMariaDB}
\end{figure}

\subsection{Mindville}
Way too small.

\clearpage
\subsection{MongoDB}
MongoDB overall has 13 link types and 37545 links.
After cleaning up link types ``Depends'' and ``Gantt Dependency'', mapping them together, we arrive at 12 link types.
We only predict on 7 of them, as ``Split'' (133), ``Backport'' (66), ``Clone'' (59), ``Test'' (48), and ``finish-finish'' (16) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on MongoDB links.}\label{tab:ResultsMongoDB}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{good} Relate       &   0.729961 &  0.712821 &  0.721289 &  3705 \\
\rowcolor{moderate} Duplicate    &   0.557960 &  0.285375 &  0.377615 &  1265 \\
\rowcolor{good} Depend       &   0.746850 &  0.404672 &  0.565236 &  1434 \\
\rowcolor{subpar} Cause        &   0.017241 &  0.206897 &  0.031830 &   116 \\
\rowcolor{good} Subtask      &   0.626761 &  0.654412 &  0.640288 &   136 \\
\rowcolor{good} Documented   &   0.750000 &  0.736527 &  0.743202 &   334 \\
\rowcolor{verygood} Epic         &   0.970787 &  0.949451 &  0.960000 &   455 \\
\hline
accuracy     &  \multicolumn{4}{r|}{0.597045} \\
macro avg    &   0.628509 &  0.571451 &  0.577066 &  7445 \\
weighted avg &   0.706616 &  0.597045 &  0.636187 &  7445 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsMongoDB} shows the result of an SVM trained on the links of the MongoDB project. 

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_mongodb_test_confmat.png}
\caption{Confusion Matrix in percent of MongoDB.}\label{fig:ConfMatMongoDB}
\end{figure}
Figure~\ref{fig:ConfMatMongoDB} shows the confusion matrix.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_mongodb_test_umap_2.png}
\caption{UMAP of the test data embeddings of MongoDB.}\label{fig:UMAPMongoDB}
\end{figure}
Figure~\ref{fig:UMAPMongoDB} shows the UMAP on the embeddings of the test set.

k-Means found 5 as the optimal number of clusters.
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_mongodb_test_ltcomp.png}
    \caption{kMeans with optimal k MongoDB}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_mongodb_test_acc_ltcomp.png}
    \caption{kMeans with accurate k MongoDB}
\end{subfigure}
\caption{kMeans of MongoDB.}\label{fig:kMeansMongoDB}
\end{figure}

\clearpage
\subsection{Qt}
Qt overall has 8 link types and 35855 links.
We only predict on 7 of them, as ``Test'' (47) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on Qt links.}\label{tab:ResultsQt}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{moderate} Duplicate    &   0.374449 &  0.343666 &  0.358398 &   742 \\
\rowcolor{good} Relate       &   0.588595 &  0.538509 &  0.562439 &  1610 \\
\rowcolor{moderate} Split        &   0.180017 &  0.407023 &  0.258294 &   477 \\
\rowcolor{good} Depend       &   0.807921 &  0.689189 &  0.743847 &  1184 \\
\rowcolor{subpar} Replace      &   0.278788 &  0.089494 &  0.135493 &   514 \\
\rowcolor{verygood} Subtask      &   0.927240 &  0.918404 &  0.922801 &  1679 \\
\rowcolor{verygood} Epic         &   0.958290 &  0.961297 &  0.959791 &   956 \\
\hline
accuracy     &  \multicolumn{4}{r|}{0.651075} \\
macro avg    &   0.587900 &  0.571083 &  0.563009 &  7162 \\
weighted avg &   0.681958 &  0.651075 &  0.657912 &  7162 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsQt} shows the result of an SVM trained on the links of the Qt project. 

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_qt_test_confmat.png}
\caption{Confusion Matrix in percent of Qt.}\label{fig:ConfMatQt}
\end{figure}
Figure~\ref{fig:ConfMatQt} shows the confusion matrix.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_qt_test_umap_2.png}
\caption{UMAP of the test data embeddings of Qt.}\label{fig:UMAPQt}
\end{figure}
Figure~\ref{fig:UMAPQt} shows the UMAP on the embeddings of the test set.

k-Means found 5 as the optimal number of clusters.
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_qt_test_ltcomp.png}
    \caption{kMeans with optimal k Qt}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_qt_test_acc_ltcomp.png}
    \caption{kMeans with accurate k Qt}
\end{subfigure}
\caption{kMeans of Qt.}\label{fig:kMeansQt}
\end{figure}

\clearpage
\subsection{RedHat}
Redhat overall has 18 link types and 106200 links.
After cleaning up link types like ``Gantt: finish-finish'' and ``finish-finish [GANTT]'', mapping them together, as well as ``Cloners'' and ``Cloners (old)'', we arrive at 14 link types.
We only predict on 8 of them, as ``Documented'' (506), ``Parent-Child'' (311), ``Split'' (104), ``finish-start'' (51), ``finish-finish'' (19), and ``start-finish'' (11) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on RedHat links.}\label{tab:ResultsRedHat}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{subpar} Cause        &   0.157171 &  0.266223 &  0.197653 &    601 \\
\rowcolor{good} Clone        &   0.781187 &  0.693297 &  0.734623 &   3342 \\
\rowcolor{good} Incorporate  &   0.831050 &  0.655013 &  0.732605 &   1945 \\
\rowcolor{good} Relate       &   0.651118 &  0.404436 &  0.555544 &   5590 \\
\rowcolor{good} Block        &   0.731061 &  0.603125 &  0.660959 &   3200 \\
\rowcolor{verygood} Subtask      &   0.930272 &  0.892709 &  0.911103 &   4334 \\
\rowcolor{subpar} Duplicate    &   0.105436 &  0.317732 &  0.158331 &   1111 \\
\rowcolor{subpar} Follow       &   0.173377 &  0.230098 &  0.197751 &    917 \\
\hline
accuracy     &  \multicolumn{4}{r|}{0.609411} \\
macro avg    &   0.545084 &  0.517829 &  0.518571 &  21040 \\
weighted avg &   0.694327 &  0.609411 &  0.642839 &  21040 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsRedHat} shows the result of an SVM trained on the links of the RedHat project. 

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_redhat_test_confmat.png}
\caption{Confusion Matrix in percent of RedHat.}\label{fig:ConfMatRedHat}
\end{figure}
Figure~\ref{fig:ConfMatRedHat} shows the confusion matrix. We observe the following:
\begin{itemize}
    \item ``Cause'' is often mistaken for ``Rleate'' and ``Duplicate'',
    \item ``Relate'' is often mistaken for ``Duplicate'' as well,
    \item ``Duplicate'' is often mistaken for ``Cause'' and ``Relate'',
    \item ``Follow''  is often mistaken for ``Cause'', ``Relate'' and ``Duplicate''.
\end{itemize}

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_redhat_test_umap_2.png}
\caption{UMAP of the test data embeddings of RedHat.}\label{fig:UMAPRedHat}
\end{figure}
Figure~\ref{fig:UMAPRedHat} shows the UMAP on the embeddings of the test set.

k-Means found 5 as the optimal number of clusters.
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_redhat_test_ltcomp.png}
    \caption{kMeans with optimal k RedHat}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_redhat_test_acc_ltcomp.png}
    \caption{kMeans with accurate k RedHat}
\end{subfigure}
\caption{kMeans of RedHat.}\label{fig:kMeansRedHat}
\end{figure}

\clearpage
\subsection{Sakai}
Sakai overall has 7 link types and 19057 links.
We only predict on 6 of them, as ``Bonfire Testing'' (1) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on Sakai links.}\label{tab:ResultsSakai}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{moderate} Depend       &   0.361032 &  0.255578 &  0.299287 &   493 \\
\rowcolor{moderate} Clone        &   0.177632 &  0.143617 &  0.158824 &   188 \\
\rowcolor{good} Relate       &   0.730259 &  0.673578 &  0.700774 &  1881 \\
\rowcolor{verygood} Subtask      &   0.896166 &  0.864407 &  0.880000 &   649 \\
\rowcolor{moderate} Duplicate    &   0.201669 &  0.415473 &  0.271536 &   349 \\
\rowcolor{moderate} Incorporate  &   0.380952 &  0.349206 &  0.364389 &   252 \\
\hline
accuracy     &  \multicolumn{4}{r|}{0.580797} \\
macro avg    &   0.407952 &  0.400310 &  0.445802 &  3812 \\
weighted avg &   0.612013 &  0.580797 &  0.591101 &  3812 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsSakai} shows the result of an SVM trained on the links of the Sakai project. 
We observe that the detection works well on ``Relate'' and ``Subtask''.
For ``Depend'', ``Clone'', ``Duplicate'', and ``Incorporate'' the detection achieves sub-par results.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_sakai_test_confmat.png}
\caption{Confusion Matrix in percent of Sakai.}\label{fig:ConfMatSakai}
\end{figure}
Figure~\ref{fig:ConfMatSakai} shows the confusion matrix.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_sakai_test_umap_2.png}
\caption{UMAP of the test data embeddings of Sakai.}\label{fig:UMAPSakai}
\end{figure}
Figure~\ref{fig:UMAPSakai} shows the UMAP on the embeddings of the test set.

k-Means found 4 as the optimal number of clusters.
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_sakai_test_ltcomp.png}
    \caption{kMeans with optimal k Sakai}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_sakai_test_acc_ltcomp.png}
    \caption{kMeans with accurate k Sakai}
\end{subfigure}
\caption{kMeans of Sakai.}\label{fig:kMeansSakai}
\end{figure}

\clearpage
\subsection{SecondLife}
SecondLife overall has 7 link types and 19057 links.
We only predict on 6 of them, as ``Bonfire Testing'' (1) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on SecondLife links.}\label{tab:ResultsSecondLife}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{verygood} Subtask      &   0.800000 &  0.923077 &  0.857143 &   52 \\
\rowcolor{good} Relate       &   0.604651 &  0.684211 &  0.641975 &   38 \\
\rowcolor{subpar} Clone        &   0 &  0 &  0 &   11 \\
\rowcolor{subpar} Depend       &   1 &  0.111111 &  0.200000 &    9 \\
\rowcolor{subpar} Parent-Child &   0.272727 &  0.214286 &  0.240000 &   14 \\
\rowcolor{moderate} Incorporate  &   0.250000 &  0.500000 &  0.333333 &    2 \\
\hline
accuracy     &  \multicolumn{4}{r|}{0.626984} \\
macro avg    &   0.407896 &  0.405447 &  0.378742 &  126 \\
weighted avg &   0.618214 &  0.626984 &  0.593596 &  126 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsSecondLife} shows the result of an SVM trained on the links of the SecondLife project. 

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_secondlife_test_confmat.png}
\caption{Confusion Matrix in percent of SecondLife.}\label{fig:ConfMatSecondLife}
\end{figure}
Figure~\ref{fig:ConfMatSecondLife} shows the confusion matrix.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_secondlife_test_umap_2.png}
\caption{UMAP of the test data embeddings of SecondLife.}\label{fig:UMAPSecondLife}
\end{figure}
Figure~\ref{fig:UMAPSecondLife} shows the UMAP on the embeddings of the test set.

k-Means found 4 as the optimal number of clusters.
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_secondlife_test_ltcomp.png}
    \caption{kMeans with optimal k SecondLife}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_secondlife_test_acc_ltcomp.png}
    \caption{kMeans with accurate k SecondLife}
\end{subfigure}
\caption{kMeans of SecondLife.}\label{fig:kMeansSecondLife}
\end{figure}

\clearpage
\subsection{Sonatype}
Sonatype overall has 11 link types and 4289 links.
We only predict on 8 of them, as ``Implements'' (11), ``Epic'' (9), ``Split'' (5) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on Sonatype links.}\label{tab:ResultsSonatype}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{moderate} Bonfire Testing &   0.292683 &  0.160000 &  0.206897 &   75 \\
\rowcolor{subpar} Duplicate       &   0.075758 &  0.089286 &  0.081967 &   56 \\
\rowcolor{good} Relate          &   0.667742 &  0.636923 &  0.651969 &  325 \\
\rowcolor{subpar} Cause           &   0.133333 &  0.038462 &  0.059701 &   52 \\
\rowcolor{moderate} Depend          &   0.290323 &  0.310345 &  0.300000 &   29 \\
\rowcolor{subpar} Supercede       &   0.088235 &  0.142857 &  0.109091 &   21 \\
\rowcolor{verygood} Subtask         &   0.863333 &  0.935018 &  0.897747 &  277 \\
\rowcolor{subpar} Fix             &   0.035714 &  0.111111 &  0.054054 &   18 \\
\hline
accuracy     &  \multicolumn{4}{r|}{0.584994} \\
macro avg       &   0.305890 &  0.303000 &  0.295178 &  853 \\
weighted avg    &   0.586403 &  0.584994 &  0.581174 &  853 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsSonatype} shows the result of an SVM trained on the links of the Sonatype project. 
We observe that the detection works well on ``Relate'' and ``Subtask''.
For ``Depend'', ``Clone'', ``Duplicate'', and ``Incorporate'' the detection achieves sub-par results.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_sonatype_test_confmat.png}
\caption{Confusion Matrix in percent of Sonatype.}\label{fig:ConfMatSonatype}
\end{figure}
Figure~\ref{fig:ConfMatSonatype} shows the confusion matrix.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_sonatype_test_umap_2.png}
\caption{UMAP of the test data embeddings of Sonatype.}\label{fig:UMAPSonatype}
\end{figure}
Figure~\ref{fig:UMAPSonatype} shows the UMAP on the embeddings of the test set.

k-Means found 4 as the optimal number of clusters.
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_sonatype_test_ltcomp.png}
    \caption{kMeans with optimal k Sonatype}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_sonatype_test_acc_ltcomp.png}
    \caption{kMeans with accurate k Sonatype}
\end{subfigure}
\caption{kMeans of Sonatype.}\label{fig:kMeansSonatype}
\end{figure}

\clearpage
\subsection{Spring}
Spring overall has 9 link types and 14461 links. 
After cleaning up link types like ``Relate'' and ``Related'', mapping them together, as well as ``Depends'' and ``Depend'', we arrive at 7 link types.
We only predict on 6 of them, as ``Clone'' (14) appeared less than 1\%.

\begin{table}
\caption{Results of SVM on Spring links.}\label{tab:ResultsSpring}
\begin{tabular}{|l|rrrr|}
\hline
Link Type &  precision &    recall &  f1-score &       support \\
\hline
\rowcolor{good} Relate       &   0.716509 &  0.769622 &  0.742116 &  1376 \\
\rowcolor{moderate} Depend       &   0.393574 &  0.275281 &  0.323967 &   356 \\
\rowcolor{verygood} Epic         &   0.977199 &  0.990099 &  0.983607 &   303 \\
\rowcolor{verygood} Subtask      &   0.861862 &  0.730280 &  0.790634 &   393 \\
\rowcolor{moderate} Duplicate    &   0.393103 &  0.158333 &  0.225743 &   360 \\
\rowcolor{subpar} Supercede    &   0.068783 &  0.254902 &  0.108333 &   102 \\
\hline
accuracy     &  \multicolumn{4}{r|}{0.632180} \\
macro avg    &   0.568505 &  0.529753 &  0.529067 &  2890 \\
weighted avg &   0.660680 &  0.632180 &  0.635832 &  2890 \\
\hline
\end{tabular}
\end{table}
Table~\ref{tab:ResultsSpring} shows the result of an SVM trained on the links of the Spring project. 

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_spring_test_confmat.png}
\caption{Confusion Matrix in percent of Spring.}\label{fig:ConfMatSpring}
\end{figure}
Figure~\ref{fig:ConfMatSpring} shows the confusion matrix.

\begin{figure}[]
\centering
\includegraphics[scale=0.40]{pictures/LT_spring_test_umap_2.png}
\caption{UMAP of the test data embeddings of Spring.}\label{fig:UMAPSpring}
\end{figure}
Figure~\ref{fig:UMAPSpring} shows the UMAP on the embeddings of the test set.

k-Means found 4 as the optimal number of clusters.
\begin{figure}[]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_spring_test_ltcomp.png}
    \caption{kMeans with optimal k Spring}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[scale=0.5]{pictures/LT_spring_test_acc_ltcomp.png}
    \caption{kMeans with accurate k Spring}
\end{subfigure}
\caption{kMeans of Spring.}\label{fig:kMeansSpring}
\end{figure}

==> tables/lt_f1_corr.tex <==
\begin{table*}[h]
\caption{EXPERIMENTAL: Correlation of F1-scores across the different link types.}\label{tab:LTCorr}
\begin{tabular}{|l|rrrrrrrrr|}
\toprule
LT &  Block &  Cause &  Clone &  Depend &  Duplicate &  Epic &  Incorporate &  Relate &  Subtask \\
\midrule
Block       &   1.00 &   1.00 &   0.66 &     NaN &      -0.49 & -0.91 &         1.00 &    0.66 &    -0.36 \\
Cause       &   1.00 &   1.00 &  -1.00 &   -0.99 &      -0.49 & -0.48 &         0.95 &    0.00 &     0.34 \\
Clone       &   0.66 &  -1.00 &   1.00 &    0.26 &      -0.93 & -0.75 &        -0.46 &   -0.77 &    -0.30 \\
Depend      &    NaN &  -0.99 &   0.26 &    1.00 &       0.18 & -0.64 &        -0.61 &    0.05 &     0.01 \\
Duplicate   &  -0.49 &  -0.49 &  -0.93 &    0.18 &       1.00 &  0.17 &        -0.39 &    0.26 &    -0.05 \\
Epic        &  -0.91 &  -0.48 &  -0.75 &   -0.64 &       0.17 &  1.00 &        -1.00 &   -0.29 &     0.65 \\
Incorporate &   1.00 &   0.95 &  -0.46 &   -0.61 &      -0.39 & -1.00 &         1.00 &    0.69 &    -0.54 \\
Relate      &   0.66 &   0.00 &  -0.77 &    0.05 &       0.26 & -0.29 &         0.69 &    1.00 &     0.08 \\
Subtask     &  -0.36 &   0.34 &  -0.30 &    0.01 &      -0.05 &  0.65 &        -0.54 &    0.08 &     1.00 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/lt_project_precision.tex <==
\begin{table*}[h]
\setlength\tabcolsep{2.5pt}  % Adjust the table column spacing
\centering
\captionsetup{skip=2pt}
\caption{Common link types across the repositories and their precision.}\label{tab:LTinRepoPrecision}
\begin{tabularx}{0.85\textwidth}{X|rrrrrrrrrr|rr}

\hline       %R   Du  S   De  E   Cl  I   C  B
\textbf{Repository} &  Relate & Duplicate & Subtask & Depend & Clone & Incorporate &  Epic & Block & Cause &  Non-Link & \textbf{Macro F1}& \textbf{Weight. F1}\\
\hline
Apache        &       \cellcolor{good}0.6 &        \cellcolor{ok}0.54 &  \cellcolor{verygood}0.89 &       \cellcolor{ok}0.51 &      \cellcolor{good}0.67 &      \cellcolor{good}0.6 &  \cellcolor{verygood}0.96 &      \cellcolor{good}0.6 &      \cellcolor{ok}0.42 &      \cellcolor{good}0.77 &       \cellcolor{good}0.6 &       \cellcolor{good}0.7 \\
Hyperledger   &      \cellcolor{good}0.68 &        \cellcolor{ok}0.56 &   \cellcolor{verygood}0.9 &           /&  \cellcolor{verygood}0.83 &           /&  \cellcolor{verygood}0.95 &     \cellcolor{good}0.65 &          /&  \cellcolor{verygood}0.84 &      \cellcolor{good}0.77 &  \cellcolor{verygood}0.84 \\
IntelDAOS     &      \cellcolor{good}0.65 &        \cellcolor{ok}0.58 &      \cellcolor{good}0.77 &           /&   \cellcolor{verygood}1.0 &           /&            /&     \cellcolor{good}0.67 &          /&      \cellcolor{good}0.62 &      \cellcolor{good}0.77 &      \cellcolor{good}0.68 \\
JFrog         &        \cellcolor{ok}0.51 &        \cellcolor{ok}0.56 &  \cellcolor{verygood}0.96 &       \cellcolor{ok}0.49 &            /&   \cellcolor{verybad}0.0 &            /&           /&          /&   \cellcolor{verygood}0.8 &        \cellcolor{ok}0.49 &      \cellcolor{good}0.66 \\
Jira          &  \cellcolor{verygood}0.85 &      \cellcolor{good}0.76 &  \cellcolor{verygood}0.94 &           /&      \cellcolor{good}0.61 &     \cellcolor{good}0.77 &            /&           /&      \cellcolor{ok}0.52 &  \cellcolor{verygood}0.87 &      \cellcolor{good}0.78 &  \cellcolor{verygood}0.82 \\
JiraEcosystem &        \cellcolor{ok}0.56 &      \cellcolor{good}0.65 &  \cellcolor{verygood}0.87 &      \cellcolor{bad}0.22 &        \cellcolor{ok}0.52 &       \cellcolor{ok}0.43 &  \cellcolor{verygood}0.96 &       \cellcolor{ok}0.42 &     \cellcolor{bad}0.39 &      \cellcolor{good}0.71 &        \cellcolor{ok}0.56 &      \cellcolor{good}0.71 \\
MariaDB       &      \cellcolor{good}0.73 &        \cellcolor{ok}0.41 &  \cellcolor{verygood}0.87 &           /&            /&     \cellcolor{good}0.68 &  \cellcolor{verygood}0.98 &     \cellcolor{good}0.69 &    \cellcolor{good}0.62 &      \cellcolor{good}0.77 &      \cellcolor{good}0.72 &      \cellcolor{good}0.71 \\
Mojang        &      \cellcolor{good}0.75 &  \cellcolor{verygood}0.96 &            /&           /&            /&           /&            /&           /&          /&  \cellcolor{verygood}0.97 &  \cellcolor{verygood}0.89 &  \cellcolor{verygood}0.95 \\
MongoDB       &      \cellcolor{good}0.69 &        \cellcolor{ok}0.51 &      \cellcolor{good}0.79 &     \cellcolor{good}0.72 &            /&           /&  \cellcolor{verygood}0.96 &           /&      \cellcolor{ok}0.49 &      \cellcolor{good}0.69 &      \cellcolor{good}0.74 &      \cellcolor{good}0.72 \\
Qt            &        \cellcolor{ok}0.51 &        \cellcolor{ok}0.49 &  \cellcolor{verygood}0.92 &     \cellcolor{good}0.76 &            /&           /&  \cellcolor{verygood}0.94 &           /&          /&   \cellcolor{verygood}0.8 &      \cellcolor{good}0.68 &      \cellcolor{good}0.71 \\
RedHat        &       \cellcolor{good}0.6 &       \cellcolor{bad}0.34 &  \cellcolor{verygood}0.87 &           /&  \cellcolor{verygood}0.84 &  \cellcolor{verygood}0.8 &            /&     \cellcolor{good}0.65 &      \cellcolor{ok}0.42 &      \cellcolor{good}0.74 &      \cellcolor{good}0.64 &       \cellcolor{good}0.7 \\
Sakai         &      \cellcolor{good}0.69 &       \cellcolor{bad}0.38 &  \cellcolor{verygood}0.89 &        \cellcolor{ok}0.5 &      \cellcolor{good}0.68 &     \cellcolor{good}0.69 &            /&           /&          /&  \cellcolor{verygood}0.81 &      \cellcolor{good}0.66 &      \cellcolor{good}0.69 \\
SecondLife    &      \cellcolor{good}0.69 &            /&  \cellcolor{verygood}0.85 &        \cellcolor{ok}0.5 &         \cellcolor{ok}0.4 &   \cellcolor{verybad}0.0 &            /&           /&          /&  \cellcolor{verygood}0.89 &        \cellcolor{ok}0.54 &      \cellcolor{good}0.73 \\
Sonatype      &      \cellcolor{good}0.67 &       \cellcolor{bad} 0.34 &  \cellcolor{verygood}0.91 &       \cellcolor{ok}0.43 &            / &           / &            / &           / &     \cellcolor{bad} 0.27 &      \cellcolor{good}0.75 &        \cellcolor{ok}0.47 &      \cellcolor{good}0.65 \\
Spring        &      \cellcolor{good}0.71 &        \cellcolor{ok}0.47 &  \cellcolor{verygood}0.83 &       \cellcolor{ok}0.43 &            / &           / &  \cellcolor{verygood}0.98 &           / &          / &      \cellcolor{good}0.73 &      \cellcolor{good}0.65 &      \cellcolor{good}0.69 \\
\hline
Mean          &      \cellcolor{good}0.66 &        \cellcolor{ok}0.54 &  \cellcolor{verygood}0.88 &       \cellcolor{ok}0.51 &      \cellcolor{good}0.69 &        \cellcolor{ok}0.5 &  \cellcolor{verygood}0.96 &     \cellcolor{good}0.61 &      \cellcolor{ok}0.45 &      \cellcolor{good}0.78 &      \cellcolor{good}0.66 &      \cellcolor{good}0.73 \\
Standard Dev. &    0.09 &    0.16 &    0.05 &   0.15 &    0.18 &       0.31 &    0.01 &   0.09 &   0.1 &    0.08 &    0.11 &    0.08 \\
\hline
\end{tabularx}
\end{table*}

==> tables/lt_project_recall.tex <==
\begin{table*}[h]
\setlength\tabcolsep{2.5pt}  % Adjust the table column spacing
\centering
\captionsetup{skip=2pt}
\caption{Common link types across the repositories and their recall.}\label{tab:LTinRepoRecall}
\begin{tabularx}{0.85\textwidth}{X|rrrrrrrrrr|rr}

\hline       %R   Du  S   De  E   Cl  I   C  B
\textbf{Repository} &  Relate & Duplicate & Subtask & Depend & Clone & Incorporate &  Epic & Block & Cause &  Non-Link & \textbf{Macro F1}& \textbf{Weight. F1}\\
\hline
Apache        &       \cellcolor{good}0.7 &        \cellcolor{ok}0.44 &  \cellcolor{verygood}0.93 &       \cellcolor{ok}0.41 &        \cellcolor{ok}0.56 &      \cellcolor{ok}0.51 &  \cellcolor{verygood}0.98 &       \cellcolor{ok}0.46 &      \cellcolor{bad}0.29 &      \cellcolor{good}0.75 &        \cellcolor{ok}0.54 &      \cellcolor{good}0.71 \\
Hyperledger   &      \cellcolor{good}0.73 &       \cellcolor{bad}0.27 &  \cellcolor{verygood}0.89 &           /&      \cellcolor{good}0.78 &          /&  \cellcolor{verygood}0.99 &       \cellcolor{ok}0.59 &           /&  \cellcolor{verygood}0.85 &      \cellcolor{good}0.73 &  \cellcolor{verygood}0.85 \\
IntelDAOS     &      \cellcolor{good}0.73 &       \cellcolor{bad}0.36 &  \cellcolor{verygood}0.87 &           /&      \cellcolor{good}0.75 &          /&            /&     \cellcolor{good}0.72 &           /&         \cellcolor{ok}0.4 &      \cellcolor{good}0.69 &      \cellcolor{good}0.68 \\
JFrog         &      \cellcolor{good}0.66 &        \cellcolor{ok}0.47 &  \cellcolor{verygood}0.94 &       \cellcolor{ok}0.41 &            /&  \cellcolor{verybad}0.0 &            /&           /&           /&      \cellcolor{good}0.66 &        \cellcolor{ok}0.47 &      \cellcolor{good}0.66 \\
Jira          &  \cellcolor{verygood}0.91 &      \cellcolor{good}0.67 &  \cellcolor{verygood}0.92 &           /&      \cellcolor{good}0.61 &      \cellcolor{ok}0.54 &            /&           /&      \cellcolor{bad}0.29 &  \cellcolor{verygood}0.85 &       \cellcolor{good}0.7 &  \cellcolor{verygood}0.83 \\
JiraEcosystem &      \cellcolor{good}0.68 &         \cellcolor{ok}0.5 &  \cellcolor{verygood}0.91 &  \cellcolor{verybad}0.16 &      \cellcolor{good}0.68 &     \cellcolor{bad}0.22 &  \cellcolor{verygood}0.99 &      \cellcolor{bad}0.39 &      \cellcolor{bad}0.36 &        \cellcolor{ok}0.53 &        \cellcolor{ok}0.52 &      \cellcolor{good}0.72 \\
MariaDB       &   \cellcolor{verygood}0.8 &       \cellcolor{bad}0.34 &  \cellcolor{verygood}0.85 &           /&            /&    \cellcolor{good}0.68 &  \cellcolor{verygood}0.96 &     \cellcolor{good}0.63 &       \cellcolor{ok}0.44 &      \cellcolor{good}0.76 &      \cellcolor{good}0.68 &      \cellcolor{good}0.72 \\
Mojang        &      \cellcolor{good}0.66 &  \cellcolor{verygood}0.97 &            /&           /&            /&          /&            /&           /&           /&  \cellcolor{verygood}0.96 &  \cellcolor{verygood}0.86 &  \cellcolor{verygood}0.95 \\
MongoDB       &      \cellcolor{good}0.76 &        \cellcolor{ok}0.42 &  \cellcolor{verygood}0.92 &     \cellcolor{good}0.66 &            /&          /&  \cellcolor{verygood}0.98 &           /&      \cellcolor{bad}0.29 &      \cellcolor{good}0.75 &      \cellcolor{good}0.71 &      \cellcolor{good}0.73 \\
Qt            &      \cellcolor{good}0.63 &       \cellcolor{bad}0.39 &  \cellcolor{verygood}0.94 &     \cellcolor{good}0.74 &            /&          /&  \cellcolor{verygood}0.97 &           /&           /&  \cellcolor{verygood}0.81 &      \cellcolor{good}0.65 &      \cellcolor{good}0.72 \\
RedHat        &      \cellcolor{good}0.67 &       \cellcolor{bad}0.25 &  \cellcolor{verygood}0.92 &           /&  \cellcolor{verygood}0.83 &    \cellcolor{good}0.74 &            /&      \cellcolor{good}0.6 &      \cellcolor{bad}0.39 &      \cellcolor{good}0.69 &      \cellcolor{good}0.61 &      \cellcolor{good}0.71 \\
Sakai         &      \cellcolor{good}0.74 &        \cellcolor{ok}0.41 &  \cellcolor{verygood}0.87 &       \cellcolor{ok}0.47 &      \cellcolor{good}0.62 &      \cellcolor{ok}0.48 &            /&           /&           /&      \cellcolor{good}0.76 &      \cellcolor{good}0.62 &      \cellcolor{good}0.68 \\
SecondLife    &      \cellcolor{good}0.78 &            /&  \cellcolor{verygood}0.89 &      \cellcolor{bad}0.33 &         \cellcolor{ok}0.4 &  \cellcolor{verybad}0.0 &            /&           /&           /&  \cellcolor{verygood}0.81 &        \cellcolor{ok}0.51 &      \cellcolor{good}0.75 \\
Sonatype      &      \cellcolor{good}0.69 &       \cellcolor{bad}0.32 &  \cellcolor{verygood}0.91 &       \cellcolor{ok}0.41 &            /&          /&            /&           /&      \cellcolor{bad}0.26 &       \cellcolor{good}0.7 &        \cellcolor{ok}0.46 &      \cellcolor{good}0.66 \\
Spring        &      \cellcolor{good}0.75 &       \cellcolor{bad}0.33 &   \cellcolor{verygood}0.8 &       \cellcolor{ok}0.54 &            / &          / &  \cellcolor{verygood}0.99 &           / &           / &      \cellcolor{good}0.75 &      \cellcolor{good}0.62 &      \cellcolor{good}0.69 \\
\hline
Mean          &      \cellcolor{good}0.73 &        \cellcolor{ok}0.44 &   \cellcolor{verygood}0.9 &       \cellcolor{ok}0.46 &      \cellcolor{good}0.65 &       \cellcolor{ok}0.4 &  \cellcolor{verygood}0.98 &       \cellcolor{ok}0.57 &      \cellcolor{bad}0.33 &      \cellcolor{good}0.74 &      \cellcolor{good}0.62 &      \cellcolor{good}0.74 \\
Standard Dev. &    0.07 &    0.18 &    0.04 &   0.16 &    0.13 &      0.27 &    0.01 &   0.11 &   0.06 &    0.13 &    0.11 &    0.08 \\
\bottomrule
\hline
\end{tabularx}
\end{table*}

==> tables/project_type.tex <==
\begin{table}[h]
\setlength\tabcolsep{2.5pt}  % Adjust the table column spacing
\centering
\captionsetup{skip=2pt}
\caption{Putting the repositories into types.}\label{tab:RepoType}
\begin{tabularx}{\columnwidth}{l X}
\hline
\textbf{Type} &     \textbf{Repositories} \\
\hline
\rowcolor{hellgrau}Hierarchical & SecondLife, JiraEcosystem, Hyperledger \\
Duplicate & Mojang \\
\rowcolor{hellgrau}Related+Causal & IntelDAOS, MariaDB, MongoDB, Sakai, Spring \\
Related+Hierarchical & Apache, JFrog, Qt, RedHat, Sonatype \\
\rowcolor{hellgrau}Related+Duplicate & Jira, Mindville\\
\hline
\end{tabularx}
\end{table}
